Efficient Algorithm for Scalable Event-based Demand Response Management in Microgrids

Demand response management has become one of the key enabling technologies for smart grids. Motivated by the increasing demand response incentives offered by service operators, more customers are subscribing to various demand response programs. However, with growing customer participation, the problem of determining the optimal loads to be curtailed in a microgrid during contingencies within a feasible time frame becomes computationally hard. This paper proposes an efficient approximation algorithm for event-based demand response management in microgrids. In event-based management, it is important to curtail loads as fast as possible to maintain the stability of a microgrid during the islanded mode in a scalable manner. A simple greedy approach is presented that can rapidly determine a close-to-optimal load curtailment scheme to maximize the aggregate customer utility in milliseconds for a large number of customers. This paper further derives a novel theoretical guarantee of the gap between the proposed efficient algorithm and the optimal solution (that may be computationally hard to obtain). The performance of algorithm is corroborated extensively by simulations with up to thousands of customers. For the sake of practicality, the proposed event-based demand response management algorithm is applied to a feeder from the Canadian benchmark distribution system. The simulation results demonstrate that the proposed approach efficiently optimizes microgrid operation during islanded mode while maintaining appropriate voltage levels and network constrains.

==> appx.tex <==
\section*{Appendix}
\begin{customthm}{1}
Algorithm ${\cA^{\rm e}}$ is\\ $\big(\frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}},1\big)$-approximation for \textsc{CKP}.
\end{customthm}
\begin{proof}
 Let $S^*=\{k^*_1,...,k^*_{s^*}\}$ and $\hat S = \{k_1,...,k_s\}$ be an optimal and the  returned solution respectively, where $|S^*| = s^*$ and $|\hat S| = s$. Also let $k_{s+1}$ denote a user with $(s+1)$-th efficiency (as ordered by Eqn.~\raf{eq:ef}). For convenience, we denote $\hat d_i \triangleq d_{k_i}$, $\hat u_i \triangleq u_{k_i}$, $ d^*_j \triangleq d_{k^*_j}$, and  $ u^*_j \triangleq u_{k^*_j}$ for $i=1,...,s$ and $j=1,...,s^*$. We first sort optimal solution $S^*=\{k^*_1,...,k^*_{s^*}\}$ by efficiency in a non-increasing order as defined in Eqn.~\raf{eq:ef}, while keeping $\hat S$ order the same.
We split the analysis into two main cases:

\noindent {\bf Case (1):} $(\hat S \cup \{k_{s+1}\}) \cap S^* = \varnothing$\\
  By the greedy order (Eqn.~\raf{eq:ef}), for every $i=1,...,s+1$ we have
 \begin{align}
 \frac{\hat u_i}{|\hat d_i|} &\ge \frac{u^*_j}{|d^*_j|} \quad \text{ for all } j = 1,...,s^*.
 \end{align}
 Using the fact that $\max_i \frac{x_i}{y_i} \ge \frac{\sum_i x_i}{\sum_i y_i}$ for any positive real numbers  $x_i,y_i$; we obtain
 \begin{align}
\frac{ \hat u_i } {|\hat d_i|}&\ge \frac{\sum_{j=1}^{s^*} u^*_j}{\sum_{j = 1}^{s^*} |d^*_j|} \iff \hat u_i  \ge \frac{|\hat d_i|}{\sum_{j = 1}^{s^*} |d^*_j|} {\sum_{j=1}^{s^*} u^*_j}.
 \end{align}
 Summing up over $i=1,...,s+1$ obtains
 \begin{align}
     \sum_{i=1}^{s+1} \hat u_i &\ge {\sum_{j=1}^{s^*} u^*_j} \frac{ \sum_{i=1}^{s+1}|\hat d_i|} {\sum_{j = 1}^{s^*} |d^*_j|}. \label{eq:g.1}
 \end{align}
 In step~\ref{alg:g.max}, the algorithm returns the maximum solution. This implies
 \begin{align}
 \max\{u(S_1), u(S_2)\} &\ge \frac{1}{2} \big( \sum_{i=1}^{s} \hat u_i + u_{\max}\big) \ge \frac{1}{2} \sum_{i=1}^{s+1} \hat u_i \nonumber\\
 & \ge \frac{1}{2}\cdot \frac{ \sum_{i=1}^{s+1}|\hat d_i|} {\sum_{j = 1}^{s^*} |d^*_j|} \OPT, \label{eq:g.2}
 \end{align}
 where $u_{\max} \triangleq \max_{k\in \cN} u_k$, and Eqn.~\raf{eq:g.2} follows by Eqn.~\raf{eq:g.1}. Finally, we bound $\frac{ \sum_{i=1}^{s+1}|\hat d_i|} {\sum_{j = 1}^{s^*} |d^*_j|}$ from below.  Since $\theta$ is at most $\frac{\pi}{2}$, and $|\sum_{i=1}^{s+1} \hat d_i | \ge C \ge |\sum_{j=1}^{s^*}  d^*_j$, we can apply Lemma~\ref{lem:tb} below and obtain: 
\begin{equation} 
\frac{ \sum_{i=1}^{s+1}|\hat d_i|} {\sum_{j = 1}^{s^*} |d^*_j|} \ge \frac{\big|\sum_{j=1}^{s^*} d^*_j \big|}{\sum_{j = 1}^{s^*} |d^*_j|}\ge \sqrt{\frac{\cos \theta + 1}{2}}. \label{eq:g.3}
 \end{equation}
 (See figure~\ref{fig:greedy} for a pictorial intuition).
\begin{figure}[!ht]
	\begin{center}
		\includegraphics[scale=0.8]{fig/fig-greedy.pdf}
	\end{center}
\caption{The figure depicts an extreme case where the ratio  $\frac{\sum_{i=1}^{s+1} |\hat d_i|}{\sum_{j = 1}^{s^*} |d^*_j|}$ is minimal. The dotted arrows represent solution $\hat S \cup \{k_{s+1}\}$ (which is in-feasible), whereas the red arrows are  optimal solution $S^*$. One can show that the two optimal sides are equal (in the extreme case). By rescaling the triangle such that each of the two optimal sides are equal to 1, $\sum_{i=1}^{s+1}|\hat d_i| \ge \sqrt{(1+\cos \theta)^2 + \sin^2 \theta} = \sqrt{2 + 2\cos \theta}$. Therefore $\frac{\sum_{i=1}^{s+1} |\hat d_i|}{\sum_{j = 1}^s |d^*_j|} \ge \frac{\sqrt{2 + 2\cos \theta}}{2}=\sqrt{\frac{\cos \theta + 1}{2}}$.}
	\label{fig:greedy}
\end{figure}  
  Combining Eqns.\raf{eq:g.2}-\raf{eq:g.3} gives
 \begin{equation}
  \max\{u(S_1), u(S_2)\} \ge \frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT. \label{eq:g.3.5}
 \end{equation}
 
\noindent {\bf Case (2):} $(\hat S \cup \{k_{s+1}\}) \cap S^* \neq \varnothing$\\
For convenience we use $i \in  S\cap S^* $, $i \in  S\backslash S^* $, $j \in S^*\backslash  S $ to indicate $k_i \in  (\hat S \cup {k_{s+1}} )\cap S^*$,  $k_i \in  (\hat S \cup {k_{s+1}} )\backslash S^*$, and  $k^*_j \in  S^*\backslash (\hat S \cup {k_{s+1}} )$ respectively.
   By the greedy order (Eqn.~\raf{eq:ef}), for every $i= S\backslash S^*$ we have
$\frac{\hat u_i}{|\hat d_i|}\ge \frac{u^*_j}{|d^*_j|} \quad \text{ for all } j \in S^*\backslash  S$.
 This implies that,
 \begin{equation}
  \frac{ \sum_{i\in  S \backslash S^*} \hat u_i}{ \sum_{i\in  S \backslash S^* }|\hat d_i|}  \ge \frac{\sum_{j \in S^*\backslash  S} u^*_j} {\sum_{j \in S^*\backslash  S} |d^*_j|}. \label{eq:g.4}
 \end{equation}

Next, if $\sum_{i\in  S \backslash S^*}  |\hat d_i| \ge \sum_{j \in S^*\backslash  S} |d^*_j|$ (by Eqn.\raf{eq:g.4}, it implies $\sum_{i\in  S \backslash S^*} \hat u_i \ge \sum_{j \in S^*\backslash  S} u^*_j$) then $\sum_{i=1}^{s+1} \hat u_i \ge \OPT$. Therefore, w.l.o.g., we assume   $\sum_{i\in  S \backslash S^*}  |\hat d_i| < \sum_{j \in S^*\backslash  S} |d^*_j|$
 
 By Lemma~\ref{lem:frac}
 \begin{align}
& \frac{\sum_{i\in  S  \cup S^*} \hat u_i +  \sum_{i\in  S \backslash S^*} \hat u_i}{ \sum_{i\in  S  \cup S^*} |\hat d_i| + \sum_{i\in  S \backslash S^* }|\hat d_i|}  \ge \frac{\sum_{i\in  S  \cup S^*} \hat u_i \sum_{j \in S^*\backslash  S} u^*_j} {\sum_{i\in  S  \cup S^*} |\hat d_i|  + \sum_{j \in S^*\backslash  S} |d^*_j|}\\
 & \sum_{i=1}^{s+1} \hat u_i \ge  \frac{ \sum_{i=1}^{s+1}|\hat d_i|} {\sum_{j = 1}^{s^*} |d^*_j|}\cdot  \OPT \ge \sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT \label{eq:g.5},
 \end{align}
 where Eqn.~\raf{eq:g.5} follow from Eqn.~\raf{eq:g.3}. The rest is similar to Eqn.~\raf{eq:g.2}-\raf{eq:g.3.5}.
 
 
 Finally, we mention that the algorithm always obtains a feasible solution (by  step~\ref{alg:g.feas} condition), the algorithm is ${\cA^{\rm e}}$ is\\ $\big(\frac{1}{2\sqrt 2} \sqrt{\cos \theta + 1},1\big)$-approximation.
\end{proof}

\medskip


\begin{lemma}
\label{lem:tb}
Given a set of 2D vectors $\{d_i \in \RR^2\}_{i=1}^n$
$$ \frac{\sum_{i=1}^n |d_i| }{\big| \sum_{i =1}^n d_i \big|} \le \sqrt{\frac{2}{\cos \theta + 1}},$$
where $\theta$ is the maximum angle between any pair of vectors and $0 \le \theta \le \frac{\pi}{2}$.
\end{lemma}
\begin{proof}
We proof $\frac{(\sum_{i=1}^n |d_i| )^2}{|\sum_{i=1}^n d_i |^2} \le \frac{\cos + 1}{2}$  by induction. First, we expand  the L.H.S.
\begin{align}
&\frac{  \sum_{i=1}^n |d_i|^2 +  2\sum_{1\le i < j \le n} |d_i| \cdot |d_j|  } { \sum_{i =1}^n |d_i|^2 +  2\sum_{1\le i < j \le n} |d_i| \cdot |d_j| (\sin \theta_i \sin \theta_j + \cos \theta_i \cos \theta_j)}\nonumber\\
&=\frac{ \sum_{i=1}^n |d_i|^2 +  2\sum_{1\le i < j \le n} |d_i| \cdot |d_j|  } { \sum_{i=1}^n |d_i|^2 +  2\sum_{1\le i < j \le n} |d_i| \cdot |d_j| \cos (\theta_i - \theta_j)}, \label{eq:ind}
\end{align}
where $\theta_i$ is the angle that $d_i$ makes with the $x$ axis.


Consider the base case: $|S|= 2$. Eqn.~\raf{eq:ind} is
\begin{align}
 \frac{|d_1|^2 +|d_2|^2 + 2 |d_1|\cdot |d_2|}{|d_1|^2 +|d_2|^2 + 2 |d_1|\cdot |d_2| \cos(\theta)} = f(x),
\end{align}
where $ f(x) \triangleq \frac{1+x^2+2x}{1+x^2+2x\cos \theta}$ and $x=\frac{|d_2|}{|d_1|}$. The first derivative $f'(x) = \frac{(1+x^2+2x \cos \theta )(2x + 2) - 1+x^2 + 2x)(2x + 2 \cos \theta)}{(1 + x^2 + 2x \cos \theta )^2}$ is zero only when $x=1$. Hence, $f(1)$ is an extreminum point.  We compare $f(1)$ with $f(x)$ at the  boundaries $x\in \{0,\infty\}$: $f(1) = \frac{2}{\cos \theta + 1} \ge f(0) = \lim_{x \to \infty} f(x) = 1$. Therefore $f(x)$ has a global maximum of $\frac{2}{\cos \theta  + 1}$.

Next we proceed to the inductive step. We assume $\frac{\sum_{i=1}^{r-1} |d_i| }{\big| \sum_{i=1}^{r-1} d_i \big|} \le \sqrt{\frac{2}{\cos \theta + 1}}$ where $r \in \{1,\ldots, n\}$. W.L.O.G., assume $\theta_1\ge\theta_3\ge \cdots \ge \theta_n \ge \theta_2$. Rewrite Eqn.~\raf{eq:ind}:
\begin{equation}
 \frac{ ( \sum_{i=1}^r |d_i|)^2 } { \displaystyle \sum_{i=1}^r |d_i|^2 + 2 \smashoperator{\sum_{1\le i<j<r}} |d_i|  |d_j| \cos (\theta_i - \theta_j) +  2 |d_r| \smashoperator{\sum_{1\le i<r}} |d_i|  \cos (\theta_i - \theta_r)}. \label{eq:den}
\end{equation}
Let $g(\theta_r)$ be the denominator of Eqn.~\raf{eq:den}. We take the  second derivative of $g(\theta_r)$:
$$g''(\theta_r) = -2 |d_r| \sum_{1 \le i < r} |d_i| \cos(\theta_i - \theta_r).$$ Notice that $\cos(\theta_i - \theta_r) \ge 0$, therefore the second derivative is always negative. This indicates that all local exterma in $[0,\theta_{r-1}]$ of $g(\theta_n)$ are local maxima. Hence, the minimum occur at the boundaries:
\begin{equation}
\min_{\theta_r \in [0,\theta_{r-1}]}  g(\theta_r) \in \{g(0), g(\theta_{r-1})\}
\end{equation}
If $\theta_r \in \{0,\theta_r\}$ there must exist at least a pair of vectors in $\{d_i\}_{i=1}^r$ with the same angle. Combining these two vectors into one, we can obtain an instance with $r-1$ vectors. Hence, by the inductive hypothesis, the same bound holds up to $r$ vectors.
\end{proof}

\medskip

\begin{lemma} 
\label{lem:frac}
Given $\frac{x}{y} \ge \frac{a_1}{b_1} \ge \frac{a_2}{b_2}$ such that  $b_1 < b_2$
$$ \frac{x+a_1}{y+b_1} \ge \frac{x+a_2}{y + b_2},$$
where $x,y,a_1,a_2,b_1$ and $b_2$ are positive real numbers.
 \end{lemma}
 \begin{proof}
 We show $\frac{x+a_1}{y+b_1} - \frac{x+a_2}{y + b_2} \ge 0 $.
 \begin{align}
 &\frac{x+a_1}{y+b_1} - \frac{x+a_2}{y + b_2}  = \frac{x(b_2 - b_1) + y(a_1 - a_2) + a_1 b_2 - a_2 b_1 }{(y+b_1)(y+b_2)} \nonumber\\
 &\ge  \frac{x(b_2 - b_1) + y(a_1 - a_2) }{(y+b_1)(y+b_2)}
 \end{align}
 We complete the proof  showing $x(b_2 - b_1) \ge   - y(a_1 - a_2)$.
 \begin{align}
 \frac{x}{y} + \frac{a_1 - a_2}{b_2 - b_1} \ge   \frac{a_1}{b_1} + \frac{a_1 - a_2}{b_2 - b_1} = \frac{a_1 b_2 - a_2 b_1}{b_1 ( b_2 - b_1)} \ge 0
 \end{align}
 \end{proof}
 


==> newresults.tex <==
\section*{New Results}\label{cha:algs}

In this chapter we present heuristic-based algorithms which were the core decision mechanisms of load curtailment DR programs examined in our study and provide theoretical guarantees on their worst-case performance. For clarity of presentation, we consider only the valuation-maximising problem. Furthermore, without loss of generality, assume $|d_k| \le C$ for all $k$ in {\sc VmaxPA} problem. An allocation $(x_k)_{k \in {\cal N}}$ can be equivalently represented by the set of satisfied customers $X \triangleq \{k\in {\cal N}\mid  x_k=1\}$. For a subset $X \subseteq {\cal N}$, we denote $u(X) \triangleq \sum_{k\in X}u_k$.

\section{Greedy Valuation Algorithm  ({\sc GVA})}

First, {\sc GVA} sorts customers in $\cN = \{1,...,n\}$ according to their valuations in a non-increasing order where ties are broken arbitrarily (i.e. equivalent candidates are selected randomly):
\begin{equation}
\label{eqn:gva}
\mbox{if\ }  k \le k', \mbox{\ then\ }  
u_{k} \ge u_{k'} \text{ for all } k,k' \in \cN.
\end{equation}
Then, {\sc GVA} obtains set $X$ by adding customers in that order until no more customers can be added without violating the capacity constraint
($\big|\sum_{k\in X}d_k x_k\big| \le C$). The pseudocode of {\sc GVA} is presented below in Algorithm \ref{alg:gva}.

\begin{algorithm}[htb!]
\caption{${\sc(GVA)} [ \{u_k,d_k\}_{k \in \cN}, C]$}
\begin{algorithmic}[1]
\Require Customers' valuations and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$
\State Sort customers in $\cN$ by their valuation defined by Equation \ref{eqn:gva}.
\State $X \leftarrow \varnothing$
\For{$k \in \cN$} 
\If{ $\big|\sum_{k' \in X} d_{k'} + d_k \big| \le C$} \label{alg:g.feas}
\State $X \leftarrow X \cup \{k\}$
\EndIf
\EndFor
\State \Return $X$
\end{algorithmic}
\label{alg:gva}
\end{algorithm}

\section{Greedy Magnitude Algorithm ({\sc GMA})}

{\sc GMA} is similar to {\sc GVA}, but sorts customers by the magnitude of their demands in a non-decreasing order:  
\begin{equation}
\label{eqn:gma}
\mbox{if\ }  k \le k', \mbox{\ then\ }  
|d_{k}| \le |d_{k'}| \text{ for all } k,k' \in \cN.
\end{equation}
Then, {\sc GMA} adds the demands in that order to solution set $X$ under consideration as long as the capacity constraint ($\big|\sum_{k\in X}d_k x_k\big| \le C$) is not violated. 

\section{Greedy Ratio Algorithm ({\sc GRA})}

Alike {\sc GVA} and {\sc GMA}, but {\sc GRA} sorts the customers by its efficiency ($\frac{u_k}{|d_k|}$) in a non-increasing order:
\begin{equation}
\label{eqn:gra}
\mbox{if\ }  k \le k', \mbox{\ then\ }  
\frac{u_k}{|d_k|} \ge \frac{u_{k'}}{|d_{k'}|} \text{ for all } k,k' \in \cN.
\end{equation}
Then, {\sc GRA} selects demands in that order until no more customers can be added without violating the capacity constraint ($\big|\sum_{k\in X}d_k x_k\big| \le C$). The pseudocode of {\sc GRA} is explained in Algorithm \ref{alg:gra}.

\begin{algorithm}[htb!]
\caption{${\sc(GRA)} [ \{u_k,d_k\}_{k \in \cN}, C]$}
\begin{algorithmic}[1]
\Require Customers' valuations and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$
\State Sort customers in $\cN$ by their efficiency ($\frac{u_k}{|d_k|}$) defined by Equation \ref{eqn:gra}.
\State $X \leftarrow \varnothing$
\For{$k \in \cN$} 
\If{ $\big|\sum_{k' \in X} d_{k'} + d_k \big| \le C$}
\State $X \leftarrow X \cup \{k\}$ 
\EndIf
\EndFor
\State \Return $X$
\end{algorithmic}
\label{alg:gra}
\end{algorithm}

\section{Greedy Duet Algorithm ({\sc GDA})}

{\sc GDA} comprises {\sc GVA} and {\sc GRA} algorithms and returns the maximum valuation of their solutions. An explicit description of {\sc GDA} is given in Algorithm \ref{alg:gda}.

\begin{algorithm}[htb!]
\caption{${\sc(GDA)} [ \{u_k,d_k\}_{k \in \cN}, C]$}
\begin{algorithmic}[1]
\Require Customers' valuations and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$
\Ensure $(\frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}},1)$-solution $X$ to \textsc{VmaxPA}
\State $X \leftarrow \varnothing$
\State $X_1 \leftarrow {\sc(GRA)}[ \{u_k,d_k\}_{k \in \cN}, C]$ 
\State $X_2 \leftarrow {\sc(GVA)}[ \{u_k,d_k\}_{k \in \cN}, C]$ 
\State Set $X \leftarrow \arg\max_{X_1, X_2}\{ u(X_1), u(X_2) \}$ \label{alg:g.max}
\State \Return $X$
\end{algorithmic}
\label{alg:gda}
\end{algorithm}

We show that {\sc GDA} in the worst case provides at least  $\frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}}$ of the optimum for {\sc VmaxPA} problem.

\begin{theorem}
Algorithm {\sc GDA} is $\big(\frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}},1\big)$-approximation for \textsc{VmaxPA}.
\label{th:gda}
\end{theorem}
\begin{proof}
We denote $Z^{\sc GDA}$ to be the valuation of the returned solution of {\sc GDA}. Let $Z^{\sc GVA}$ and $Z^{\sc GRA}$ be the valuation of the returned solution {\sc GVA} and {\sc GRA} respectively, for the {\sc VmaxPA} problem. Let $ S^\ast = \{d_1^{\ast},...,d_m^{\ast}\} \subseteq {\cal N}$ be an optimal solution of {\sc VmaxPA}, and the $\OPT \triangleq \sum_{k \in  S^\ast} u_k$ be the corresponding total valuation.
 
If we substitute customers' complex-valued power demand in the {\sc VmaxPA} problem by its real-valued magnitude and relax the binary decision variable $x_k$ such that it takes non-negative real values instead of only integers values (i.e. $(x_k)_{k \in {\cal N}} \in [0, 1]^n$) we get the following linear programming (LP) problem

\begin{eqnarray}
\textsc{(LVmaxPA)} \qquad& \displaystyle \max_{x_k \in [0, 1]} \sum_{k\in{\cal N}}u_k x_k \label{LVmaxPA}\\
\text{subject to}\qquad & \displaystyle \sum_{k\in {\cal N}}|d_k| x_k \le C. \label{C2}
\end{eqnarray}

We denote by $ S^\ast_{L} \subseteq {\cal N}$ an optimal solution of {\sc LVmaxPA} and by $\OPT_L \triangleq \sum_{k \in  S^\ast_{L}} u_k$ the corresponding total valuation. In chapter 2 of \cite{KPP10book} it was proved that the optimal solution to {\sc LVmaxPA} problem can be determined easily, since the problem admits the greedy choice property. In other words, a global optimum of the problem can be achieved by choosing a series of locally optimal choices. The greedy choice for {\sc LVmaxPA} problem is to select customers in sorted order defined by Equation \ref{eqn:gra}. Assume at some iteration $t$ adding the next customer to the solution set causes capacity constraint violation, that is

\begin{equation}
\displaystyle \sum\limits_{k=1}^{t-1} |d_k| \le C \text{ and } \sum\limits_{k=1}^{t} |d_k| > C.
\end{equation}

The greedy execution is stopped at this point and the remaining capacity $C - \sum\limits_{k=1}^{t-1} |d_k|$ is occupied by the corresponding fractional part of the $t$-th customer's power demand. Let $ \hat{p} \triangleq \sum\limits_{k=1}^{t-1} u_k $ and $u_{\max} \triangleq \max_{k\in \cal N} u_k$. It was also proved in \cite{KPP10book} that

\begin{equation}
\label{eq:optl}
\displaystyle \OPT_L \le \hat{p} + u_{\max}.
\end{equation}

Evidently, $Z^{\textsc {GRA}} \ge \hat{p}$ and $Z^{\textsc {GVA}} \ge u_{\max}$. This gives

\begin{equation}
\label{eq:optl2}
\displaystyle \OPT_L \le Z^{\sc GRA} + Z^{\sc GVA}.
\end{equation}

On the other hand, from Lemma \ref{lem:tb} we know that

\begin{equation}
\displaystyle \sqrt{\frac{\cos \theta + 1}{2}} \cdot \sum_{i \in S^\ast} |d_i^{\ast}| \le \Big| \sum_{i \in S^\ast} d_i^{\ast} \Big | \le C
\end{equation}

\noindent since we restrict $\theta$ to be at most $\frac{\pi}{2}$. Notice that the subset $S^{\ast}$ becomes a feasible solution to {\sc LVmaxPA} if we set the relaxed decision variable $x_i=\sqrt{\frac{\cos \theta + 1}{2}}$ for $\forall i \in S^{\ast}$ and $x_i=0$ otherwise. This implies that

\begin{equation}
\label{eq:optl4}
\displaystyle \OPT_L \ge \sqrt{\frac{\cos \theta + 1}{2}} \cdot u(S^{\ast}) = \sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT.
\end{equation}

By {\sc GDA} formulation $Z^{\sc GDA} \ge Z^{\sc GRA}$ and $Z^{\sc GDA} \ge Z^{\sc GVA}$, hence from Equations \ref{eq:optl2} and \ref{eq:optl4} we obtain

\begin{equation}
\label{eq:optl5}
\displaystyle Z^{\sc GDA}  \ge \frac{1}{2} \sqrt{\frac{\cos \theta + 1}{2}} \OPT.
\end{equation}
\end{proof}
In a practical setting of power systems as well as in our experiments the maximum phase angle $\theta$ between any pair of demands is restricted to be in $[0, 36^{\circ}]$\cite{NEC}. This implies that $\sqrt{\frac{\cos \theta + 1}{2}} > 0.95$. Thus {\sc GDA} is capable to obtain at least $\frac{9}{19}$-approximation for {\sc VmaxPA} problem only in $\mathcal{O}(|\cN|log{} |\cN|)$ time. 

\section{Greedy Strive Algorithm ({\sc GSA})}\label{secgsaalg}

{\sc GSA}, initially, considers the highest cumulative valuation among all the possible sets of customers whose size is smaller than $m$, where $m$ depends on the input parameter of {\sc GSA}  $\epsilon \in (0,1)$. Particularly it iterates through all the possible sets of customers of size $m$. If the cumulative demand of the set does not violate the capacity then {\sc GSA} applies {\sc GDA} on the joint set of two subsets. The first subset incorporates the latter set of customers determined prior to applying {\sc GDA}, while the second subset comprises the remaining customers possessing only smaller valuation than the minimum valuation among customers in the first subset. Particularly, {\sc GDA} is applied to the second subset only but considering demands of all the customers in the first subset. In other words, regardless of the decision made by {\sc GDA} regarding the second subset of customers, all the customers in the first subset are already included in the solution. A more comprehensive description of {\sc GSA} is provided in Algorithm \ref{alg:gsa}.

\begin{algorithm}[htb!]
\caption{${\sc(GSA)} [ \{u_k,d_k\}_{k \in \cN}, C, \epsilon]$}
\begin{algorithmic}[1]
\Require Customers' valuations and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$; $\epsilon$
\Ensure $(1-\epsilon)\sqrt{\frac{\cos \theta + 1}{2}}$-approximation solution $S$ for \textsc{VmaxPA}
\State $m \leftarrow \arg\min \{\ceil {\frac{1}{\epsilon}}-2, |\cN|\}$
\State $S \leftarrow \varnothing$
\For {$\textbf{all } \text{subsets } \hat{S} \subset{\cN} \text{ such that } |\hat{S}| < m$} 
\If{ $\big|\sum_{k \in \hat{S}} d_{k}\big| \le C$}
\If{ $u(\hat{S}) \ge u(S)$}
\State $S \leftarrow \hat{S}$ 
\EndIf
\EndIf
\EndFor

\For {$\textbf{all } \text{subsets } \hat{S} \subset{N} \text{ such that } |\hat{S}| = m$} 
\If{ $\big|\sum_{k \in \hat{S}} d_{k}\big| \le C$}
\State  $L \triangleq{\{j|j \in \cN, u_j \le \min_{i \in \hat{S}} u_i \} \setminus \hat{S}} $
\State $S_1 \leftarrow {\sc(GDA)}[ \{u_k,d_k\}_{k \in L \cup \hat{S}}\text{, such that  } x_i = 1 \text{ for } \forall i \in \hat{S}, C]$
\If{ $u(S_1) \ge u(S)$}
\State $S \leftarrow S_1$ 
\EndIf
\EndIf
\EndFor
\State \Return $S$
\end{algorithmic}
\label{alg:gsa}
\end{algorithm}


\begin{theorem}
Algorithm {\sc(GSA)} is $(1-\epsilon)\sqrt{\frac{\cos \theta + 1}{2}}$-approximation for \textsc{VmaxPA}.
\end{theorem}
\begin{proof} We extend the proof provided in \cite{KPP10book} for real-valued demands. Let us denote by $Z^{\sc GSA}$ the valuation of the returned solution of {\sc GSA}. Also, we denote by $ S^\ast = \{d_1^{\ast},...,d_m^{\ast}\} \subseteq {\cal N}$ an optimal solution of {\sc VmaxPA} and by $\OPT \triangleq \sum_{k \in  S^\ast} u_k$ the corresponding total valuation. In the case when $\OPT$ comprises a a subset of customers with cardinality smaller than $m$ then, evidently, {\sc GSA} returns optimum solution. Alternatively, consider a subset of customers $\bar{S} \subseteq S^{\ast}$ with length $m$ that contributes the most in the optimal solution. {\sc GSA} determines this during its execution and executes {\sc GDA} on the joint set of $\bar S$ and the remaining customers in set $S' \triangleq{\{j|j \in \cN, u_j \le \min_{i \in \bar S} u_i \}} \setminus \bar S$. We denote by $Z_{S'}^{\sc GDA}$ the valuation of the returned solution of {\sc GDA} on the subset of customers $S'$ and also set $\OPT_{S'}$ to be the valuation of the optimal solution for that subset. From the formulation of {\sc GSA} we have that $Z^{\sc GSA} \ge u(\bar S) + Z_{S'}^{\sc GDA}$. We also have that $\OPT = u(\bar S) + \OPT_{S'}$. We split the analysis into two main cases:\\
\noindent {\bf Case (1):} $u(\bar S) \ge \frac{m}{m+2} \sqrt{\frac{\cos \theta + 1}{2}} \OPT$.

We know from Theorem \ref{th:gda} that $Z_{S'}^{\sc GDA} \ge \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT_{S'}$. From the aforementioned we get 

\begin{eqnarray}
\displaystyle & Z^{\sc GSA} &\ge u(\bar S) + \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT_{S'} \\
\displaystyle & & \ge u(\bar S) + \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} (\OPT - u(\bar S))\\
\displaystyle & & \ge u(\bar S)(1- \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}}) + \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT.
\label{eq:gsa1}
\end{eqnarray}

From the condition of this case and Equation \ref{eq:gsa1}  we immediately obtain

\small{
\begin{eqnarray}
\displaystyle & Z^{\sc GSA} &\ge \frac{m}{m+2} \sqrt{\frac{\cos \theta + 1}{2}} \OPT (1- \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}})  + \\ &&\frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT \\
\displaystyle && \ge \frac{m}{2(m+2)} \sqrt{\frac{\cos \theta + 1}{2}} \OPT + \frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT\\
\displaystyle & & = \OPT \sqrt{\frac{\cos \theta + 1}{2}} (\frac{m}{2(m+2)} + \frac{1}{2})\\
\displaystyle & & = \OPT \sqrt{\frac{\cos \theta + 1}{2}} (\frac{2m+2}{2(m+2)})\\
\displaystyle & & = \OPT \cdot \frac{m+1}{m+2} \sqrt{\frac{\cos \theta + 1}{2}}. \label{eq:gsa2} 
\end{eqnarray}
}
 Since $\frac{m+1}{m+2}$ increases with $m$, considering the value of $m$ we obtain
 
 \begin{equation}
 \displaystyle Z^{\sc GSA} \ge \OPT \cdot \frac{\frac{1}{\epsilon}-1}{\frac{1}{\epsilon}} \sqrt{\frac{\cos \theta + 1}{2}} \ge (1-\epsilon) \sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT.
 \end{equation}

\noindent {\bf Case (2):} $u(\bar S) < \frac{m}{m+2} \sqrt{\frac{\cos \theta + 1}{2}} \OPT$.\\
The condition on this case requires that at least one customer in set $\bar S$ should have a valuation less than $\frac{1}{m+2} \sqrt{\frac{\cos \theta + 1}{2}}\OPT$. From the problem formulation we have that customers in set $S'$ should have valuation smaller than $\frac{1}{m+2}\sqrt{\frac{\cos \theta + 1}{2}}\OPT$. Recall Theorem \ref{th:gda} where we show that 

\begin{equation}
\label{eq:gsa3}
\displaystyle \sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT_{S'} \le \OPT^L_{S'} \le Z_{S'}^{\sc GDA} + u_{\max}^{S'}
\end{equation}

\noindent where $u_{\max}^{S'} \triangleq \max_{k\in S'} u_k$ and $\OPT^L_{S'}$ is the optimal solution of subset of customers $S'$ for the relaxed LP. Considering that $u_{\max}^{S'} \le \frac{1}{m+2}\sqrt{\frac{\cos \theta + 1}{2}}\OPT$ and the way we formulated the optimal solution set we get

\begin{eqnarray}
\displaystyle & \OPT \cdot \sqrt{\frac{\cos \theta + 1}{2}} & \le u(\bar S) \cdot \sqrt{\frac{\cos \theta + 1}{2}} + Z_{S'}^{\sc GDA} + \\ &&\frac{1}{m+2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT \\
\displaystyle & & \le Z^{\sc GSA} + \frac{1}{m+2}\sqrt{\frac{\cos \theta + 1}{2}} \OPT.
\label{eq:gsa4}
\end{eqnarray}

By rewriting Equation \ref{eq:gsa4} we obtain

\begin{equation}
\displaystyle Z^{\sc GSA} \ge \OPT \sqrt{\frac{\cos \theta + 1}{2}}(1 - \frac{1}{m+2}) \ge \sqrt{\frac{\cos \theta + 1}{2}}\frac{m+1}{m+2} \cdot \OPT.
\end{equation}

This implies that

\begin{equation}
\displaystyle Z^{\sc GSA} \ge (1-\epsilon)\sqrt{\frac{\cos \theta + 1}{2}} \cdot \OPT.
\end{equation}
\end{proof}
Thus, we have shown for both cases that {\sc GSA} is an $(1-\epsilon)\sqrt{\frac{\cos \theta + 1}{2}}$-approximation for {\sc VmaxPA} for any $\epsilon \in [0,1]$. Recall that in a practical setting and in our experiments $\sqrt{\frac{\cos \theta + 1}{2}} > 0.95$. Hence {\sc GSA} can achieve at least $(1-\epsilon) 0.95$ of the optimum solution in $\mathcal{O}({|\cal N|}^{\frac{1}{\epsilon} -1}log{} |\cN|)$ time. 


\section{Customer Valuation/Compensation Function}

Customer cost function is a key consideration when designing demand management contracts \cite{918305,747493} and could be a subject of a separate thesis. Each customer in SG is an individual entity and makes independent decisions on his/her energy consumption and preferences. To model customers preferences we define a valuation function $u_k(|d_k|)$ for each customer $k \in {\cal N}$ which indicates the amount of money that customer $k$ is willing to pay for receiving $|d_k|$ units of energy. Similarly, we define customer compensation function $c_k(|d_k|)$ which indicates the amount of money that customer $k$ is paid if not supplied by $|d_k|$ units of energy. We make the following assumptions for the valuation and compensation functions (for clarity consider only valuation function):

\begin{enumerate}

\item \label{assum1} The valuation function is increasing based on the consumed energy capacity. In other words, for each $k \in {\cal N}$, we have
\begin{equation}
\displaystyle  {u_k}({|d_k|}) \le {u_k}({{|d'_k|}}), \text{  }\forall\text{ } {|d_k|} \le {{|d'_k|}}.
\end{equation}
\item \label{assum2} The valuation function is strictly convex. For each  $k \in {\cal N} $, any $0 \le \alpha \le 1$, and ${|d_k|},{|d'_k|} \ge 0$, we have
\begin{equation}
\displaystyle  u_k(\alpha |d_k| + (1 - \alpha)|d'_k|) < \alpha \cdot u_k(|d_k|) + (1 - \alpha)u_k(|d'_k|).
\end{equation}
\item \label{assum3} When the consumption level equals to zero
\begin{equation}
\displaystyle u_k(|d_k|) = 0 \text{  }\forall\text{ } |d_k| = 0.
\end{equation}

\end{enumerate}

Quadratic functions are among a number of practical examples of valuation/compensation functions \cite{6266724, 5628271} that satisfy the aforementioned Assumptions \ref{assum1}, \ref{assum2} and \ref{assum3}. We adopt the following quadratic function as customer valuation and compensation function
\begin{equation}
\label{eq:valuationfunction}
\displaystyle  c_k({|d_k|}) = u_k({|d_k|}) = a({|d_k|})^2 + b{|d_k|} + c
\end{equation}
where $a > 0$ and $b, c \ge 0$ are pre-determined constants. In addition to this compensation/valuation scheme we also consider several special cases, which are discussed in the proceeding sections.  


\section{Data Set}

Since the required data for our experiments may be confidential and is not publicly available, we generate artificial data set of customers considering diverse scenarios in the aspects of power demands, load types and valuations/compensations. The list of scenarios is detailed below. 


\begin{itemize}
\item{ Power demands:}
\begin{itemize}
\item {\em Full (F) power}: Each customer's power demand comprises both non-negative active power ($P_k \ge 0$) and non-negative reactive power ($Q_k \ge 0$).

\item {\em Active (A) power only}: Each customer's power demand comprises non-negative active power ($P_k \ge 0$) but zero reactive power ($Q_k = 0$). 
\end{itemize}

\item{Valuation/Compensation-demand correlation:}
\begin{itemize}
\item {\em Correlated (C)}: Each customer's valuation and compensation are a function of the power demand and are defined by (\ref{eq:valuationfunction}).
\item {\em Uncorrelated (U)}: Each customer's valuation and compensation are independent of the power demand and are randomly selected from $(0, D]$ and $(0, W)$ respectively, where $D, W > 0$ are positive constants.
\item {\em Linear (L)}: Each customer's valuation and compensation are determined by the following equation

\begin{equation}
\displaystyle  c_k({|d_k|}) = u_k({|d_k|}) = m({|d_k|}) + z
\end{equation}
where $m, z > 0$ are pre-determined values. Within the same type of customers these values are same among all customers. However, they may be different among customers belonging to different types.

\end{itemize}

\item {Load types:}

\begin{itemize}

\item {\em Residential (R) customers}: Customers have small demands ranging from 500VA to 8KVA.

\item {\em Industrial (I) customers}: Customers have big demands ranging from 500KVA up to 2MVA.

\item {\em Mixed (M) customers}: MG contains a mix of industrial and residential customers. 

\end{itemize}

\end{itemize}


In the proceeding, we represent a scenario by the acronyms
of the types. For instance, scenario ACR corresponds to the one with zero reactive power demands, correlated valuations/compensations with demands and only residential customers. 


\section{Experiments on a Single Link Distribution System MG} \label{cha:experiment1}

Having a comprehensive investigation of power allocation problems in MGs with a single link distribution system and corresponding DR algorithms assured with a precise worst-case guarantee on the optimality gap and well-defined research objectives, we analyse the running time and quality of the returned solution of the explored algorithms through extensive simulations. We further provide the findings of comparison between the algorithms considering the solution returned by GUROBI optimiser as a baseline for comparison. The performed experiments include diverse scenarios with regards to customer types, compensation/valuation correlation, generation profile and power demands. We applied {\sc GVA}, {\sc GMA}, {\sc GDA}, {\sc GSA} and {\sc GRA} to {\sc VmaxPA} problem and the accordingly modified versions of {\sc GVA}, {\sc GMA}, {\sc GDA} and {\sc GRA} to {\sc CminPA} problem. The value of $\epsilon$ for {\sc GSA} was set to be $\frac{1}{4}$ in the scenarios with mixed industrial and residential customers and $\frac{1}{3}$ in the scenarios with only residential customers unless otherwise stated. The generated customers' data sets in the experiments were random. Thus we repeated experiments independently for every specified number of customers more than 30 times. We compare and interpret the results using confidence interval (CI), which defines the reliability of an estimate of the outcome. In correspondence with the practical regulations executed in power systems that require customers to conform to a certain maximum power factor $\frac{P_k}{|d_k|} \ge 0.8$ \cite{NEC}, we restrict the maximum phase angle between any pair of demands to be in the range of $[0, 36^{\circ}]$ in all the experiments.

Under the baseline conditions, we empirically show that {\sc GSA} is the most superior algorithm in terms of returned valuation for {\sc VmaxPA} problem as compared to candidate greedy algorithms. With respect to run-time we show that {\sc GDA} is more preferable for both {\sc VmaxPA} and {\sc CminPA} problems among the considered algorithms. For {\sc CminPA} problem, we illustrate through extensive simulations that {\sc GDA} is more efficient when it comes to minimising compensation compared to the candidate algorithms. To sum up, we observed that when applied to {\sc VmaxPA} and {\sc CminPA} the proposed {\sc GSA} and {\sc GDA} are far more preferable in terms of both worst-case guarantee and empirical ratio with the optimum than GVA and GMA, which are common strategies of load curtailment in practice. For {\sc VmaxPA} problem the latter algorithms may perform arbitrarily bad than the optimal solution, whereas the proposed ones have well defined approximation ratios. Moreover, experiments corroborate the explicit dominance of {\sc GSA} and {\sc GDA} over {\sc GMA} and {\sc GVA} for both problems. The aforementioned implies that when designing a decision mechanism for an event-based DR program a utility company may consider employing {\sc GSA} for maximising the total valuation but should carefully consider the available time for the operation. When required to make an immediate decision {\sc GDA} may be adopted for both valuation-maximising and compensation-minimising objectives. Furthermore, one may consider adopting a hybrid approach, that is a two-stage event-based DR algorithm. In order to assure MG stable operation as a result of sudden demand imbalance, the first stage utilises {\sc GDA}, capable of obtaining a near-optimal solution, to determine the load to be curtailed in microseconds base. The second stage relies on {\sc GSA} that can further improve the optimality of the solution of the first stage up to nearly the optimum by decreasing the input value of $\epsilon$, when more response time is permitted.

\section{Valuation-maximising Power Allocation Problem}
In this section we present a detailed discussion regarding the performance of {\sc GVA}, {\sc GMA}, {\sc GDA}, {\sc GSA} and {\sc GRA} when applied to {\sc VmaxPA} problem in terms of running time and maximised valuation. We refer to the returned solution of the GUROBI optimiser for {\sc VmaxPA} problem as {\sc GUROBI OPT MAX}. We consider two main settings for {\sc VmaxPA} problem in MGs with single link distribution system, namely static capacity and dynamic capacity, which are described previously. In each setting we consider diverse scenarios in order to obtain a comprehensive and unbiased performance comparison of the candidate algorithms. We experimentally show that {\sc GDA} and {\sc GSA} are capable of determining close-to-optimal solutions, especially the latter. When it comes to run-time simulations demonstrate that {\sc GDA} is advantageous, since, unlike {\sc GSA}, it requires only milliseconds to be executed. 


\subsection{Results and Analysis}

This section scopes the analysis and discussion of the experimental results of the candidate algorithms mentioned previously when applied to {\sc VmaxPA} problem for an MG with a single link distribution system. In general, we observed that the performance of the algorithms is strongly affected by three key factors, namely the correlation between customers valuation and demand, maximum phase angle $\theta$ and range of customers' apparent power. The worst-case guarantee of {\sc GSA} with input value $\epsilon=\frac{1}{4}$ or $\epsilon=\frac{1}{3}$ outperforms that of {\sc GDA}. Even though a superior worst-case guarantee does not necessarily imply superior empirical ratio, however, empirical results corroborate dominance of {\sc GSA} over {\sc GDA} and the remaining greedy algorithms. The empirical analysis revealed that the most profitable algorithm, for {\sc VmaxPA} problem in both static and varying capacity settings, in terms of maximised valuation was {\sc GSA} followed by {\sc GDA}. Nonetheless, {\sc GSA} pays for the quality of solution by its running time. Experiments indicate that {\sc GDA} is far more efficient in terms of run-time compared to {\sc GSA}. One may observe from the formulation of {\sc GDA} that it is guaranteed to terminate in $\mathcal{O}(|\cal N|\log{}|\cal N|)$. Whereas, {\sc GSA} has a running time complexity in order of $\mathcal{O}(|\cN|^{\frac{1}{\epsilon}-1}log{}|\cal N|)$. Remarkably high empirical ratio of {\sc GSA} and relatively lower one of {\sc GDA} are partially attributed to the fact that in our experiments maximum phase angle $\theta$ between any pair of demands is upper bounded by $36^{\circ}$. 

\subsubsection{Maximised Valuation} \label{sec:maximval}

A summary of the simulation results for each scenario in the static capacity setting is presented in Tables \ref{algsstaticmax1} and \ref{algsstaticmax2}. Specifically, six scenarios are highlighted in Figures \ref{vmaxpa1}, \ref{vmaxpa2} and \ref{vmaxpa3}. Under the conditions and assumptions made, {\sc GSA} was superior compared to other greedy algorithms in terms of maximised valuation in almost all the considered scenarios. In fact, the solution returned by {\sc GSA} was significantly close to the optimum returned by GUROBI optimiser as could be observed from Figures \ref{vmaxpa1}, \ref{vmaxpa2} and \ref{vmaxpa3}. This confirms the theoretical guarantees obtained previously in Section \ref{secgsaalg}.


\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/aum-flm}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA}, {\sc GSA} and {\sc GMA} apply to {\sc VmaxPA} for scenarios AUM and FLM on left and right respectively.}
\label{vmaxpa1}
\end{figure} 


Overall performance of {\sc GDA} was slightly worse compared to {\sc GSA} but sufficiently better compared to other greedy algorithms. {\sc GDA} returns the the maximum valuation of two candidate solutions: either the solution by {\sc GRA}, or by {\sc GVA}. Simulations illustrate that, basically, if one of the candidates fails to generate a solution with close-to-optimal valuation the other, in spite, succeeds. Specifically, Figures \ref{vmaxpa1} and \ref{vmaxpa2} support the aforementioned claim. This explains the relatively good performance of {\sc GDA}. Nonetheless, in some cases both {\sc GRA} and {\sc GVA} may not produce a solution with high valuation. This may happen when considering scenarios with only few industrial customers with large demands, which practically are very unlikely for small MGs.  

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{F}} \\ \cline{2-4} 
 & \textbf{C} & \textbf{U} & \textbf{L} \\ \hline
\multicolumn{1}{|c|}{\textbf{R}} & \begin{tabular}[c]{@{}c@{}}\{GVA, GRA, GVA\},\\ GSA, GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GSA, GDA, GRA\},\\ GVA, GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}GSA, \{GDA, GRA, \\ GMA\}, GVA\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{M}} & \begin{tabular}[c]{@{}c@{}}\{GSA, GVA, GDA, \\ GRA\},GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GSA, GDA, GRA\}, \\ GMA, GVA\end{tabular} & \begin{tabular}[c]{@{}c@{}}GSA, \{GDA, GRA\},\\ GMA, GVA\end{tabular} \\ \hline
\end{tabular}
\caption{The results of experiments for {\sc VmaxPA} problem in each scenario with full power in static capacity setting. Each cell of the table indicates the performance order of the candidate algorithms from best to worst in the corresponding scenario. Algorithms in curly braces have same, very close or complementary performance ratio.}
\label{algsstaticmax1}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{}} & \multicolumn{3}{c|}{\textbf{A}} \\ \cline{2-4} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{C}} & \multicolumn{1}{c|}{\textbf{U}} & \multicolumn{1}{c|}{\textbf{L}} \\ \hline
\multicolumn{1}{|l|}{\textbf{R}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\{GDA, GRA, GVA\},\\  GSA, GMA\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\{GSA, GDA, GRA\}, \\ GVA, GMA\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}GSA, \{GDA, GRA, \\ GMA\}, GVA\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\textbf{M}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\{GSA, GVA, GDA,\\  GRA\}, GMA\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\{GSA, GDA, GRA\},\\ GMA, GVA\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}GSA,\{GMA, GDA, \\ GRA\}, GVA\end{tabular}} \\ \hline
\end{tabular}
\caption{The results of experiments for {\sc VmaxPA} problem in each scenario with active power only in static capacity setting. Each cell of the table indicates the performance order of the candidate algorithms from best to worst in the corresponding scenario. Algorithms in curly braces have same, very close or complementary performance ratio.}
\label{algsstaticmax2}
\end{table}

In the scenarios with only residential customers the difference between the valuations of the returned solutions by {\sc GRA} and {\sc GVA} may be notably close as illustrated in Figures \ref{vmaxpa2} and \ref{vmaxpa3}. This is because the customers loads are significantly smaller compared to the overall capacity and the customers demands' range is small. On the other hand, when considering scenarios with mixed customers the performance of these algorithms and difference between the results may alter dramatically since the criteria of selecting large industrial customers with demands as large as nearly half of the generation capacity may vary among {\sc GSA} and {\sc GDA} depending on scenarios. This could be inferred from Figures \ref{vmaxpa1} and \ref{vmaxpa2}.

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/alm-fcr}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA}, {\sc GSA} and {\sc GMA} apply to {\sc VmaxPA} for scenarios ALM and FCR on left and right respectively.}
\label{vmaxpa2}
\end{figure} 

We also observed a remarkable difference in performance of algorithms for scenarios with different type of correlation between customer valuation and demand. When considering a quadratic valuation function {\sc GDA} and {\sc GSA}, generally, perform well and return close-to-optimal solutions, especially in scenarios with residential customers. Both, {\sc GSA} and {\sc GRA}, firstly, include industrial customers in the solution, since their valuation to demand ratio is higher compared to residential customers. When there are enough residential customers the returned valuation of these algorithms is more or less close to the optimum as shown in Figure \ref{vmaxpa2}. The same performance ratio is observed for scenarios with customers' demands not correlate with valuations. In this case, {\sc GMA} and {\sc GVA} fail to produce high valuation. This is because, when customers' valuation is random selecting customers according to their valuation or magnitude may not be a beneficial strategy. Unlike the scenarios with quadratic valuation function, where industrial customers' valuation is exponentially bigger than that of residential ones, in those with linear valuation function the difference between industrial and residential customers' valuation is only linear. Thus, it is more likely that selecting numerous residential customers would be more beneficial than choosing an industrial customer with large valuation. This explains the superior performance of {\sc GRA} and {\sc GSA} compared to {\sc GVA}. When considering scenarios with uncorrelated valuations and demands, {\sc GRA} is far more superior compared to {\sc GVA}. This is mainly because {\sc GVA} firstly includes in the solution customers with high valuation without taking into account their power demands. For example, {\sc GVA} may select an industrial customer which has a high valuation and a considerably big demand. Other residential customers posessing relatively small valuation but significantly small demand may be ignored by {\sc GVA}. Whereas, {\sc GRA} considers the valuation to apparent power ratio when selecting customers, which is more beneficial for this case. 

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/fur-aur}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA}, {\sc GSA} and {\sc GMA} apply to {\sc VmaxPA} for scenarios FUR and AUR on left and right respectively.}
\label{vmaxpa3}
\end{figure} 

Simulations indicate that the performance of {\sc GSA} and {\sc GDA} may be affected by the maximum phase angle $\theta$ as well. More precisely, the smaller the $\theta$ the higher the valuations of the returned solutions. When considering active power demands (i.e. $\theta = 0$) empirical ratio of {\sc GSA} and {\sc GDA} is higher compared to the case with full power demands. The latter observation can be seen from Figure \ref{vmaxpa3}. This is in correspondence with the theorethical results, since when $\theta = 0$ {\sc GSA} and {\sc GDA} worst-case guarantees are $(1-\epsilon) \OPT$ and $\frac{\OPT}{2}$ respectively. Particularly, for these scenarios {\sc GSA} is a PTAS for {\sc VmaxPA} problem.


\subsubsection{Running Time}

In this section we present empirical analysis of run-time for {\sc GDA} and {\sc GSA} with different $\epsilon$ input values when applied to {\sc VmaxPA}. With increasing customer participation the running time of the algorithms increases as Figure \ref{vmaxpa7} shows. Empirical results support the theoretical results for {\sc GSA} and {\sc GDA} on termination guarantee discussed previously. Despite, the fact that GUROBI optimiser, sometimes, executes faster than {\sc GSA}, however, it does not yield any guarantees on termination. In other words, it is likely that the optimiser will not terminate in a feasible time for some problem instances. The optimiser allows to define termination criteria manually. However, in our experiments even with the relaxed termination criteria adopted, which were presented before, we observe that GUROBI optimiser fails to terminate or return an answer from time to time. Henceforth, we do not consider and analyse its running time. 

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/running_time_vmaxpa}
	\end{center} 
\caption{The running time of {\sc GDA} and {\sc GSA}.}
\label{vmaxpa7}
\end{figure} 

As Figure \ref{vmaxpa7} depicts, {\sc GDA} is far more superior in terms of running time compared to {\sc GSA} in both cases when $\epsilon = \frac{1}{4}$ and $\epsilon = \frac{1}{3}$. {\sc GDA} is capable of returning at least $\frac{1}{2}\sqrt{\frac{\cos \theta + 1}{2}}$ of the optimum in milliseconds, whereas the former requires seconds and even minutes. Also, we observe that unlike {\sc GDA} which running time increases more or less the same pace with respect to the increase in number of customers, the rate of growth of the run-time of {\sc GSA} changes at much higher rate with higher customer participation. This is supported by Figure \ref{vmaxpa7}. 

\section{Compensation-minimising Power Allocation Problem}

A thorough analysis is being considered in this section on the performance of correspondingly modified versions of {\sc GVA}, {\sc GMA}, {\sc GDA} and {\sc GRA} for {\sc CminPA} problem. We evaluate the candidate algorithms with respect to the returned minimised compensation and the running time. The modified version of {\sc GVA} sorts customers according to their valuations opposite to the order defined in Equation \ref{eqn:gva}, that is in a non-decreasing order. Then curtails the demands in that order until the remaining customers' demands do not violate the capacity constraint. Similarly, the according versions of {\sc GMA} and {\sc GRA} sort customers in inverse order of Equations \ref{eqn:gma} and \ref{eqn:gra} respectively, then continue similar to {\sc GVA} and return the cumulative compensation of customers whose load was shed. The adapted version of {\sc GDA} returns the minimum compensation of two candidate solutions: either solution by {\sc GVA} or by {\sc GRA}. We denote by {\sc GUROBI OPT MIN} the returned solution of the GUROBI optimiser for {\sc CminPA} problem. As for {\sc VmaxPA}, here also we examine settings with static capacity and dynamic capacity. For obtaining more reliable results we analyse the performance of the algorithms in various scenarios. {\sc VmaxPA} and {\sc CminPA} intuitively are similar and one may mistakenly assume that the same theoretical guarantees hold for {\sc GSA} and {\sc GDA} for the latter problem. Despite the absence of the guarantee on the worst-case performance of {\sc GDA}, we empirically illustrate that the algorithm obtains near-optimal solutions for {\sc CminPA} problem. In general, for this problem {\sc GDA} is the most preferable algorithm in terms of minimised compensation among other candidate algorithms. Moreover, we show that the difference between the running time of {\sc GDA} and {\sc GMA} is negligible. 

\subsection{Results and Analysis}

In this section we discuss the experimental results of the comparison between the considered algorithms for {\sc CminPA} problem in an MG with a single link distribution system. As for the maximisation problem, for this problem as well the correlation between customers' valuation and demand, maximum phase angle $\theta$, and range of customers' apparent power are the major factors that impact the performance of algorithms. If for {\sc VmaxPA} problem the higher the returned valuation the more preferable is the algorithm, for {\sc CminPA} problem, in contrast, the lower the returned compensation the more profitable is the algorithm. The results of experiments revealed the explicit superiority of {\sc GDA} over {\sc GVA}, {\sc GRA} and {\sc GMA}. In both, static and dynamic settings, the returned compensation by {\sc GDA} was significantly close to the optimum returned by GUROBI optimiser. Whereas, {\sc GMA} in some scenarios generated as worse as three times higher compensation than GUROBI optimiser. The only desirable property of {\sc GMA} in contrast to {\sc GDA} was its running time. However, since the difference is remarkably small it is safe to assume that {\sc GDA} is the most superior algorithm for {\sc CminPA} problem among candidates in both criteria.

\subsubsection{Minimised Compensation}

Tables \ref{algsstaticmin1} and \ref{algsstaticmin2} introduce a synopsis of the experimental results for each scenario in the static capacity setting. We highlight six scenarios in Figures \ref{vminpa1}, \ref{vminpa2} and \ref{vminpa3}. Under the conditions employed {\sc GDA} outperformed the other greedy algorithms in terms of minimised compensation in all the considered scenarios. As could be seen from Figures \ref{vminpa1}, \ref{vminpa2} and \ref{vminpa3} the empirical ratio of {\sc GDA} with respect to {\sc GUROBI OPT MIN} approaches one. 


\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/min-acr-fcr}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA} and {\sc GMA} apply to {\sc CminPA} for scenarios ACR and FCR on left and right respectively.}
\label{vminpa1}
\end{figure} 


Generally, we observe that the performances of {\sc GMA} and {\sc GVA} are complementary. When {\sc GMA} fails to minimise the compensation {\sc GVA} succeeds and vice versa. The latter claim is supported by Figures \ref{vminpa3} and \ref{vminpa2}. Experiments indicate that superior performance of {\sc GDA} is due to {\sc GRA}, which unlike {\sc GVA} performed well in all the scenarios. For {\sc CminPA} problem, {\sc GRA} may fail in situations when there are few residential customers whose compensation-to-demand ratio is high and several industrial customers with large demands and relatively lower compensation to demand ratio. Given the aforementioned set of customers, {\sc GRA} would firstly curtail demands of large industrial customers, thus generating high compensation. Since this is unlikely to occur practically in small MGs, our experiments do not capture this scenario.   

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{F}} \\ \cline{2-4} 
 & \textbf{C} & \textbf{U} & \textbf{L} \\ \hline
\multicolumn{1}{|c|}{\textbf{R}} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GVA\},\\  GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GMA\},\\  GVA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GMA, GRA, GDA\},\\  GVA\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{M}} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GVA\},\\  GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA\}, \\ GMA,GVA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA\},\\  GMA,GVA\end{tabular} \\ \hline
\end{tabular}
\caption{The results of experiments for {\sc CminPA} problem in each scenario with full power only in static capacity setting. Each cell of the table indicates the performance order of the candidate algorithms from best to worst in the corresponding scenario. Algorithms in curly braces have same, very close or complementary performance ratio.}
\label{algsstaticmin1}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{A}} \\ \cline{2-4} 
 & \textbf{C} & \textbf{U} & \textbf{L} \\ \hline
\multicolumn{1}{|c|}{\textbf{R}} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GVA\},\\  GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA\},\\  GVA, GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GMA, GRA, GDA\},\\  GVA\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{M}} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GVA\},\\  GMA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GMA\}, \\ GVA\end{tabular} & \begin{tabular}[c]{@{}c@{}}\{GRA, GDA, GMA\},\\  GVA\end{tabular} \\ \hline
\end{tabular}
\caption{The results of experiments for {\sc CminPA} problem in each scenario with active power only in static capacity setting. Each cell of the table indicates the performance order of the candidate algorithms from best to worst in the corresponding scenario. Algorithms in curly braces have same, very close or complementary performance ratio.}
\label{algsstaticmin2}
\end{table}

Similar to the maximisation problem, here also, it could be inferred from the experimental results that the performance ratios of {\sc GRA}, {\sc GVA} and {\sc GMA} change among scenarios with different load types. As could be observed from Figure \ref{vminpa3} {\sc GMA} returns almost three times higher compensation in the scenario with mixed industrial and residential customers than in the one with only residential customers. For {\sc CminPA}, again, we observe the same dependence of the results on the maximum phase angle $\theta$. When considering scenarios with active power only, the candidate algorithms return comparatively closer to optimal compensation than in the scenarios with full power. This observation is confirmed in Figure \ref{vminpa2}.   

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/min-aur-fur}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA} and {\sc GMA} apply to {\sc CminPA} for scenarios AUR and FUR on left and right respectively.}
\label{vminpa2}
\end{figure} 

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.4]{images/min-flm-flr}
	\end{center} 
\caption{{\sc GVA}, {\sc GDA}, {\sc GRA} and {\sc GMA} apply to {\sc CminPA} for scenarios FLM and FLR on left and right respectively.}
\label{vminpa3}
\end{figure} 

Additionally, empirical results revealed that the correlation between customers' demands and compensation may affect the performance of explored algorithms significantly. Figure \ref{vminpa1} depicts that for the scenarios with quadratic compensation function {\sc GMA} is far worse compared to {\sc GVA}. The converse situation occurs for the scenarios with linear compensation function as shown in Figure \ref{vminpa3}. The reason behind this behaviour of {\sc GMA} and {\sc GVA} is discussed in details previously in Section \ref{sec:maximval}.

\subsubsection{Running Time}

In this section we introduce the results of experiments for the running time of {\sc GMA} and {\sc GDA} when applied to {\sc CminPA} problem. From theoretical point of view, the run-time for both algorithms is in order of $\mathcal{O}(|\cN|\log{}|\cal N|)$. We experimentally show that {\sc GMA} outperforms {\sc GDA}, nonetheless, the latter terminates only milliseconds later than the former. In general, the higher the number of customers the higher the required running time for the candidate algorithms to terminate as shown in Figure \ref{vminpa7}. For {\sc CminPA} problem, again, we do not analyse the running time of GUROBI optimiser since the same behaviour is observed as for {\sc VmaxPA} problem. 

\begin{figure}[!ht]
	\begin{center} 
		\includegraphics[scale=.6]{images/runningtimemin}
	\end{center} 
\caption{The running time of {\sc GDA} and {\sc GMA}.}
\label{vminpa7}
\end{figure}


